The shooting algorithm for partially control-affine problems with application to an SIRS epidemiological model

In this article we propose a shooting algorithm for partially-affine optimal control problems, this is, systems in which the controls appear both linearly and nonlinearly in the dynamics. Since the shooting system generally has more equations than unknowns, the algorithm relies on the Gauss-Newton method. As a consequence, the convergence is locally quadratic provided that the derivative of the shooting function is injective and Lipschitz continuous at the optimal solution. We provide a proof of the convergence for the proposed algorithm using recently developed second order sufficient conditions for weak optimality of partially-affine problems. We illustrate the applicability of the algorithm by solving an optimal treatment-vaccination epidemiological problem.

==> DifferentialAlgebraic.tex <==

The Pontryagin Maximum Principle implies that the optimal state function $\xh$ together the multiplier $\ph$ are solutions of a {\em two-point boundary value problem} (TPBVP) induced by equations \eqref{state.dynamics}, \eqref{initial-final.constraints}, \eqref{costate_dynamics} and \eqref{transversality.conditions}, when we use \eqref{stationarity.Hamiltonian} to write the controls as functions of $x$ and $p$. The first step is \deleted{to find} \joao{to show that} such representation of the controls \deleted{that will be discussed next} \joao{exists}.

We use the stationarity of the Hamiltonian, \eqref{stationarity.Hamiltonian}, together with a suitable strengthened version of the Legendre-Clebsch condition to write the system in the form
\begin{equation}
\tag{IFTsys}
\label{IFTsys}
	\begin{split}
	\Theta(\xi, \alpha) &= 0,\\
	D_{\alpha}\Theta(\xi, \alpha) &\succ 0.
	\end{split}
\end{equation}
In this general system \eqref{IFTsys}, $\alpha$ and $\xi$ play the role of the controls $(u,v)$ and the tuple $(x, p)$, respectively. After a system as \eqref{IFTsys} is assembled, the {\em Implicit Function Theorem} (IFT) is applied to find a representation of $\alpha$ in terms of $\xi$.

\subsection{Controls in feedback form}
The conventional Legendre-Clebsch condition assumes the form 
\begin{equation}
	\label{LegendreClebsch.mixed}
	\tag{LC}
	 \left(
	 \begin{array}{cc}
	 	H_{uu}[\hat\lambda](\wh) & H_{uv}[\hat\lambda](\wh)\\
	 	\\
	 	
	 	H_{vu}[\hat\lambda](\wh)
	 	 & H_{vv}[\hat\lambda](\wh)
	 \end{array}
	 \right)
	 \succeq 0.
\end{equation}
A proof of \eqref{LegendreClebsch.mixed} for the present setting can be found in {\em e.g.} Aronna \cite[Corollary 1]{aronna2017second}. Note that, since $H_{vv}[\lambda](\wh) = 0$, condition \eqref{LegendreClebsch.mixed} holds if, and only if 
\begin{equation}
	\label{LegendreClebsch.mixed.equivalent}
	H_{uu}[\lambda](\wh) \succeq 0 \text{ and } H_{uv}[\lambda](\wh) = 0.
\end{equation}
Since the matrix in \eqref{LegendreClebsch.mixed} is singular we cannot apply the IFT to obtain our desired representations of the controls. Instead, we resort to the time derivatives of the {\em switching function}, $H_v$.
  
In order to compute the required time derivatives, consider a vector field $F:\mathbb{R}^n \times \mathbb{R}^m \to \mathbb{R}^n$  and let us evaluate the time derivative of the scalar function $\ph \cdot F(\xh, \uh)$
\begin{equation}
\label{aux}
	\begin{split}
		\disp \frac{\dd}{\dd t}&(\ph \cdot F(\xh, \uh)) 
		= \disp  
		\dot{\ph}\cdot F(\xh, \uh) + \ph \cdot D_x F(\xh, \uh) \dot{\xh} + \ph \cdot D_u F(\xh, \uh) \dot{\uh}\\
	& = \disp   
		\ph \cdot\left( D_x F f_0 - D_x f_0F + \sum_{i = 1}^m \vh_i \left(  D_x Ff_i - D_x f_iF\right) \right) + \ph \cdot D_u F \dot{\uh}.
	\end{split}
\end{equation}

It is advantageous to introduce the definition of {\em Lie brackets}. Given two differentiable vector fields $g,h:\mathbb{R}^n \to \mathbb{R}^n$ the {\em Lie bracket} is defined by
\begin{equation}
\label{Lie.Brackets}
[g,h] := D_x h(x)g(x) - D_x g(x)h(x).
\end{equation}
We use the same notation for functions depending on other variables as well, however the jacobians are taken only w.r.t. $x$. \deleted{Using the new introduced notation, \eqref{aux} becomes} \joao{This way, \eqref{aux} becomes}
\begin{equation}
\label{genericvectorfield.D1}
\frac{\dd}{\dd t}(\ph \cdot F(\xh, \uh)) = \ph \cdot [f_0, F] + \sum_{i = 1}^m \vh_j \ph \cdot [f_i, F] + \ph \cdot D_u F \dot{\uh}.
\end{equation}
We obtain \deleted{the first time derivative of $H_{v_i}$} \joao{$\dot{H}_{v_i}$}, by choosing $F = f_i$ so that, recalling $H_{vu}=0$, \deleted{equation \eqref{genericvectorfield.D1} becomes} \joao{we get}
\begin{equation}
\label{switching.function.D1_preview}
\dot{H}_{v_j}[\hat\lambda](\wh) = \ph \cdot [f_0, f_j] + \sum_{i = 1}^m \vh_j \ph \cdot [f_i, f_j].
\end{equation}
\deleted{The difficulties arise from the fact that \eqref{genericvectorfield.D1} does not depend explicitly of the linear controls.} \joao{We still can not retrieve $(u,v)$ since, in fact, \eqref{genericvectorfield.D1} does not depend explicitly of the linear controls.} This is a consequence of the following proposition which is a corollary of second order necessary conditions for optimality when the set of multipliers is a singleton, as it is our case in virtue of Assumption \ref{qualification.constraints}. 
\begin{proposition}[Goh conditions]
	\label{Goh.condition}
	Assume that $\wh(\cdot)$ is a weak minimum. Then the following identities hold
	\begin{equation*}
	\ph \cdot [f_i, f_j](\cdot) \equiv 0, \quad \text{ for $i,j = 1, \cdots, m$}.
	\end{equation*}
\end{proposition} 

Proposition \ref{Goh.condition} was first introduced by Goh, and was further generalized to this context by Aronna in \cite[Cor. 5.2]{aronna2017second} (see also \cite{aronna2012quadratic} and \cite{frankowska2013pointwise}). Equation \eqref{switching.function.D1_preview} reduces to
\begin{equation}
\label{switching.function.D1}
\dot{H}_{v_i}[\hat\lambda](\wh) = \ph \cdot [f_0, f_i].
\end{equation}
We now compute the second time derivative, applying again \eqref{genericvectorfield.D1}, this time choosing $F =  [f_0, f_i]$. We obtain
\begin{equation}
\label{hamiltonian_2timedev}
	\ddot{H}_{v_i} = \ph \cdot \left[f_0,  [f_0, f_i]\right]+\sum_{j = 1}^m \vh_j \ph \cdot \left[f_j,  [f_0, f_i]\right] + \ph \cdot D_u[f_0, f_i]\dot{\uh}.
\end{equation} 
Provided that the singular controls do not vanish in \eqref{hamiltonian_2timedev}, we must remove the dependence on $\dot{\uh}$. This can be done by using the stationarity condition $H_u[\lambda](\wh) = 0$. Assuming enough regularity, the total time derivative of this expression gives
\begin{equation}
\label{H_udot}
\dot{H}_u[\hat\lambda](\wh) = H_{ux}[\hat\lambda](\wh) \dot{\xh} + H_{up}[\hat\lambda](\wh) \dot{\ph} + H_{uu}[\hat\lambda](\wh) \dot{\uh} + H_{uv}[\hat\lambda]\dot{v}= 0,
\end{equation}
\joao{where the term $H_{uv}[\hat\lambda]\dot{v}$ vanishes because of \eqref{LegendreClebsch.mixed.equivalent}.}To formalize \eqref{H_udot}, we make the following assumption on the controls.
\begin{assumption}[Regularity of the controls]
	\label{regularity.controls}
	The nonlinear control $\uh(\cdot)$ is continuously differentiable and the linear control $\vh(\cdot)$ is continuous. 
\end{assumption}
This assumption is not restrictive since it follows from the IFT, once we assume the strengthened generalized Legendre-Clesbch condition, \eqref{LC-like.mixedcontrols} below. \deleted{The term $H_{uv}[\hat\lambda]\dot{v}$ vanishes from \eqref{LegendreClebsch.mixed.equivalent}, hence we do not require further regularity for $v$.} \joao{We do not require differentiability for $v$, since the coefficient of $\dot{v}$ vanishes}. Using the last equation and assuming the strengthened Legendre-Clebsch condition for $u$, {\em i.e.} $H_{uu}\succ 0$, we can lose the dependence of $\dot{\uh}$. Taking $\Theta = \dot{H}_u$, by \eqref{H_udot}, system \eqref{IFTsys} becomes
\begin{equation}
\dot{H}_u = 0, \quad 
H_{uu} \succ 0.
\end{equation}
Applying the IFT we get the following representation of $\dot{\uh}$
\begin{equation}
\label{representation.nonlin.derivative}
\dot{\uh} = \Gamma(\uh, \vh, \xh, \ph),
\end{equation}
where $\Gamma$ is a $\C^1$ function.

Equation \eqref{representation.nonlin.derivative} shows that the dependence on $\dot{\uh}$ can be dropped from \eqref{hamiltonian_2timedev}. Therefore we are in position to formulate a system that can be used to achieve our desired representation.
Consider the mapping
\begin{equation}
	\label{somemapping}
	(w, \lambda) \mapsto
	\left(\begin{array}{cc}
		H_u[\lambda](w)\\
		\\
		-\ddot{H}_v[\lambda](w)
	\end{array}\right).
\end{equation}
In order to obtain a formulation such as in \eqref{IFTsys} once more, we assume the derivative of mapping \eqref{somemapping} w.r.t. $(u,v)$ satisfies the {\em Strengthened Legendre-Clesbch condition} at the extremal $(\wh, \hat\lambda)$
\begin{equation}
\label{LC-like.mixedcontrols}
\tag{SLC}
	\J :=
	\left(\begin{array}{cc}
	\disp
	H_{uu}[\hat \lambda](\wh) & H_{uv}[\hat \lambda](\wh) \\
	& \\
	\disp
	-\frac{\partial \ddot{H}_v}{\partial u}[\hat \lambda](\wh) &\disp  -\frac{\partial \ddot{H}_v}{\partial v}[\hat \lambda](\wh)
	\end{array}\right) \succ 0.
\end{equation}
Once again, we are in position to apply (IFT) and retrieve the controls.

\begin{proposition}[Elimination of the controls]
	\label{control.elimination}
	If $\wh$ is a weak solution for problem (OC), provided that equation \eqref{LC-like.mixedcontrols}, then one has the representation
	\begin{equation}
	\label{control.elimination.equation}
		\uh = U(\xh, \ph) \quad \vh = V(\xh, \ph),
	\end{equation}
	where $U$ and $V$ are smooth functions of the states and costates.
\end{proposition}

From the previous discussion, we can write our optimal control problem as a Two Point Boundary Value Problem (TPBVP), which is often called the optimality system and is stated in the following theorem. 

\begin{theorem}
	\label{OC-OSequivalence}
	Under \ref{LC-like.mixedcontrols}, if $\wh$ is a {\em weak minimum} with associated multiplier $\hat\lambda$, then $(\wh, \hat\lambda)$ satisfy the following {\em optimality system}
	\begin{equation}
	\label{optimality.system}
	\tag{OS}
	\left\{\begin{array}{ll}
	\disp
	\dot{x} = f(x,U(x,p), V(x,p)), &\text{ a.e. on $[0,T],$}\\
	\\
	\disp
	\dot{p} = -p\cdot D_xf(x,U(x,p), V(x,p)), &\text{ a.e. on $[0,T],$}\\
	\\
	\eta_j(x(0), x(T)) = 0, &\text{ for } j = 1, \cdots, d_{\eta},\\
	\\
	p(0) = -D_{x_0}\ell[\lambda](x(0), x(T)),&\\
	\\
	p(T) = D_{x_T}\ell[\lambda](x(0), x(T)),&\\
	\\
	H_v(x(T), U(x(T), p(T))) = 0, &\\
	\\
	\dot{H}_v(x(0), U(x(0), p(0))) = 0. &\\
	\end{array}\right.
	\end{equation}
\end{theorem}
The stationarity of the Hamiltonian is implied by the substitution of the controls from Proposition \ref{control.elimination} and boundary conditions $H_v(T) = \dot{H}_v(0) = 0.$

\input{linear_cont_linear_sys.tex}




==> SIRS.tex <==
In this section we follow the discussion in \cite{gaff2009optimal, ledzewicz2011optimal} of the optimal control of variations of the SIR model, used to describe the dynamics of spread for a general epidemic in some demographic population.

One of the simplest attempts to control such epidemic is to include a control term $v$ modelling vaccination of susceptible individuals $S$, leading them to the recovered class $R$ before they enter the infected class $I$, and the treatment of the infected is modelled by a second control term $u$. This model is suitable for diseases for which the individuals can not suffer more than one infection. Hence, the SIRS model takes into account the effect of temporary immunity of recovered individuals, but gradually reintroduces them into the susceptible class. We shall use the following ODE
\begin{equation}
\label{NSI}
\begin{array}{rl}
\dot{N} &= F(N) - \delta I - \mu N\\
\dot{S} &= F(N) - \beta \frac{IS}{N} -vS + \omega (N - S - I) - \mu S\\
\dot{I} &= \beta \frac{IS}{N} - (\gamma + \delta + u)I - \mu I,
\end{array}
\end{equation}

In equation \eqref{NSI}, instead of using the traditional states $S,I,R$, we introduce the total number of individuals in the population, $N = S + I + R$. Working with the variables $(N,S,I)$ simplifies the computations, as done in \cite{gaff2009optimal, ledzewicz2011optimal}. The function $F:[0,K) \to \mathbb{R}_+$ is the population growth function. We assume the logistic growth model, {\em i.e.} $F(N) = \alpha N(1 - N/K)$ and that all newborn individuals enter the susceptible class.

Our goal is to minimize the amount of diseased individuals with the lowest cost with vaccination and treatment over a time window, hence we choose the following cost function
\begin{equation}
	\label{cost_function_SIR}
	\int_{0}^{T} \left(B_1 I(t) + B_2v(t) + B_3u^2(t) \right)\dd t 
\end{equation}

The choice of terms $B_1I$ and $B_3u^2$ follows \cite{gaff2009optimal}, the integral of the former is proportional to the total amount of deaths due to the disease, while the former is chosen to model the difficulty of public health agents to implement treatment strategies to a wide portion of the population. Vaccination on the other hand is more easily implemented  and hence appears linearly in the cost as in \cite{ledzewicz2011optimal}. The linear dependence on the vaccination might result in bang-bang optimal controls as in \cite{behncke2000optimal}, however the parameters values in Table \ref{Parameter table} were chosen to favor the appearance of singular arcs.

==> SIRS_OC.tex <==
Now we introduce the optimal control problem in Mayer form
\begin{equation}
	\label{SIR_problem}
	\begin{array}{cl}
		\text{minimize} & C(T) \\
		\text{subject to} & \dot{N} = F(N) - \delta I - \mu N,\\
		&\dot{S} = F(N) - \beta \frac{IS}{N} -vS + \omega (N - S - I) - \mu S, \\
		&\dot{I} = \beta \frac{IS}{N} - (\gamma + \delta + u)I - \mu I,\\
		&\dot{C} = B_1I + B_2v + B_3u^2,\\
		& 0\le v(t) \le v_{max}, \quad \text{a.e. on $[0,T]$}\\
		& 0\le u(t) , \quad \text{a.e. on $[0,T]$}\\
		& N(0) = N_0, \quad S(0) = S_0, \quad I(0) = I_0, \quad C(0) = 0.
	\end{array}
\end{equation}

We will show that the restriction on the nonlinear controls is redundant, since a "negative treatment" is never optimal. This is intuitive since negative treatment values would introduce more infected individuals to the overall population, and therefore increase the cost.
\begin{proposition}
	An optimal treatment strategy $\uh$ for problem \eqref{SIR_problem} will never present negative values.  
\end{proposition}
\begin{proof}
	Suppose an optimal solution $(\uh, \vh)$ is such that $\uh(t)$ presents negative values in a measurable set. Define a new control strategy, where $\vh$ remains unchanged and exchange $\uh$ by $u_0 := \max\{\ub, 0\}$. The cost associated with $\vh$ is unaffected, the term depending on the treatment, $\int_{0}^{T}u^2(s)\dd s$, is clearly less expensive for $u_0$ and it remains to be checked the influence on the cost associated with the amount of infected individuals of this strategy. 
	
	With this in mind, let $(N,S,I)$ and $(N_0, S_0, I_0)$ be the solutions for \eqref{NSI} with the control strategies $(\uh, \vh)$ and $(u_0, \vh)$, respectively. To conclude our argument, it suffices to show that the quantity $z:= I_0 - I$ is non positive. Note that
	\begin{align*}
		\dot{I}_0 - \dot{I} = \beta I_0 \frac{S_0}{N_0} - \beta I \frac{S}{N} - (\gamma + \delta + \mu)(I_0 - I) + \uh I\chi_{\{\uh < 0\}}.
	\end{align*}
	Hence, we can define a continuous function $c(t)$, depending on $S_0, N_0, S, N$, such that
	\begin{equation*}
		\dot{z} \le \left(\beta c(t) - \left(\gamma + \delta + \mu + \uh \xi_{\{\uh >0\}} \right)\right)z + \uh I\chi_{\{\uh < 0\} }.
	\end{equation*}
	Defining the functions $a(t) := \beta c(t) - \left(\gamma + \delta + \mu + \uh \chi_{\{\uh >0\}} \right)$ and $b(t) := \uh I\chi_{\{\uh < 0\} }$, by Gronwall's lemma, we have that
	\begin{equation*}
		z(t) \le z(0)\exp\left(\int_{0}^t a(s) \dd s\right) + \int_{0}^{t}b(s)\exp\left(\int_{0}^s a(\sigma) \dd \sigma\right)\dd s.
	\end{equation*}
	However, by definition $z(0) = 0$ and $b \le 0$, it follows that $I_0 \le I$. 
\end{proof}

The singular vaccination strategies are obtained using the expression for $\ddot{H}_v$ derived in \eqref{kernel_equation.prev1}. The complete analytical computation can be found in appendix \ref{appendix}; however, our computational implementation relies on SymEngine - a CAS (Computer Algebra System), see \cite{certiksymengine} - to automate this laborious task and other computations necessary to formulate our algorithm.

We employed the Shooting algorithm proposed in the present work to solve the optimal control problem \eqref{SIR_problem}. We used the BOCOP software \cite{bonnans2012bocop} to get an estimate of the shooting parameters and initialize our algorithm. 

\begin{figure}[h!]
	\centering
	\includegraphics[width=1.6\linewidth, center]{figs/SIR_Control_trajectories.eps}\\
	\indent 
	\caption[]{Optimal trajectories for problem \eqref{SIR_problem}.}
	\label{trajectories}
\end{figure} 

\begin{figure}[h!] 
	\indent{\centering\includegraphics[width=1.6\linewidth, center]{figs/SIR_Control_controls.eps}}\\
	\indent 
	\caption[]{Optimal controls for problem \eqref{SIR_problem}.}
	\label{controls}
\end{figure} 
 
\begin{table}[!h]
	\centering
	%\begin{tabular}{l{2.5cm}c{8cm}c{3cm}r{2.5cm}}
	\begin{tabular}{cll}
		\hline
		{\bf Parameter} & {\bf Biological Meaning} & {\bf Values} \\
		\hline
		\hline
		$N_0$    & Initial total population       & 5000 humans    \\
		$S_0$    & Initial susceptible population & 4500 humans    \\
		$I_0$    & Initial infected population    & 499  humans    \\
		$\alpha$ & Population growth rate         & $4. 10^{-5}$ / day  \\
		$K$      & Carrying capacity              & 5000           \\
		$\mu$    & Natural death rate of population & $10^{-5}$ / day  \\
		$\beta$  & incidence rate                 & 0.5 / day      \\
		$\omega$ & waning rate                    & 0.01 / day     \\
		$\gamma$ & infection time                 & 0.1 / day      \\ 
		$\delta$ & death rate due to disease      & 0.1 / day      \\
		$B_1$    & Cost per death                 & 1              \\
		$B_2$    & Cost per vaccination           & 50             \\
		$B_3$    & Cost per treatment             & 1000           \\
		$v_{max}$& Maximum vaccination rate  	  & 0.25       \\
		$T$      & Period of analysis      		  & 100 days       \\
		\hline
	\end{tabular}
	\caption{Biologically feasible parameter ranges}
	\label{Parameter table}
\end{table}


==> ShootingConvergence.tex <==










==> control_constraints_test.tex <==
In this section we extend the proposed algorithm to problems where the controls are bounded. We consider restrictions of the form

\begin{equation}
	\label{constraint.control}
	\begin{array}{c}
			(u(t), v(t)) \in U\times V, \text{ a.e. on $[0,T]$,}\\
			\text{$U\times V$ is a compact rectangle in $\mathbb{R}^l \times \mathbb{R}^m$ }.			 
	\end{array}
\end{equation}
For simplicity, consider $U\times V = [0,1]^l\times [0,1]^m$.
    
We will denote by (CP), the problem formed by (OC) and the control restrictions \eqref{constraint.control}. Given some $i = 1, \cdots, l$ the control $u_i$ is said to have a bang arc in a interval $I$, of non zero measure, if $u_i(t) = 0$ or $u_i(t) = 1$ a.e. on this interval, otherwise, it has a singular arc iff the control assumes the values $0$ and $1$ at most in a null measure set on such interval. Analogously for $v_j$ we define the same convention.

%$0\le u_i(t) \le 1$ a.e. on this interval\footnote{Assumes the values $0,1$ in a null Lebesgue measure set.}. 

Whenever a component of $u$ or $v$ switches from a singular to a bang arc, or vice verse, at a time $t \in (0, T)$, it will be called a {\em switching time}.

Our strategy to prove the convergence of the shooting algorithm in this setting will be to start considering the case where the control sets are open and limitted. This way, given the knowledge of the structure of the bang-singular arcs, we will be able to map the contrained problem to a transformed one, that is unconstrained, where a Pontryagin minimum of the latter will be mapped into a weak minimum of the former. Afterwards, we will extend this result to compact constraint sets.

\subsection{Open contraint sets}
We begin with a simpler case where the constraint sets are of the form 
\begin{equation*}
	U = (-\rho, 1 + \rho)^l, \ \ V = (-\rho, 1 + \rho)^m,
\end{equation*}
with $\rho > 0$, and consider the following assumption.
\begin{assumption}
	\label{number_switchs}
	Each component of $\uh$ and $\vh$ is a finite concatenation of bang and singular arcs. Equivalently, the optimal solution has a finite number of switching times.
\end{assumption}

From Assumption \ref{number_switchs} we can consider a partition of the time interval $[0,T]$ given by the switching times
\begin{equation*}
\{0 := \Th_0 < \Th_1 < \Th_2 < \cdots < \Th_{N-1} < \Th_N := T\}. 
\end{equation*}
Set the intervals $\Ih_k := [\Th_{k-1}, \Th_k]$, for $k = 1, \cdots, N$ and define the following set of indexes
{
\color{red}
\begin{equation*}
	\begin{array}{c}
		S_k^{\alpha} := \{ 1\le i \le l: \bar\alpha_i \text{ is singular on }\Ih_k \} \\
		E_k^{\alpha} := \{ 1\le i \le l: \bar\alpha_i = 0 \text{ a.e. on }\Ih_k \} \\
		N_k^{\alpha} := \{ 1\le i \le l: \bar\alpha_i = 1 \text{ a.e. on }\Ih_k \}, 
	\end{array}
\end{equation*}
for $\alpha \in \{u,v\}$.\footnote{These sets are not clear when we consider controls in an open set. This is the only short coming of this approach that I see. Can we get around it?}
}
\begin{assumption}
	\label{LC-constrained}
	For each $k = 1, \cdots, N$, denote by $u_{S_k}$ the vector with components $u_i$ with $i \in S_k^u$, analogously for $v_{S_k}$. In the interval $\Ih_k$ we assume the following form of the Legendre-Clesbch conditions
	\begin{equation*}
		\begin{array}{cc}
		\disp \frac{\partial^2}{\partial u_{S_k}^2}H \succ 0, & \disp -\frac{\partial }{\partial v_{S_k}}\ddot{H}_{v_{S_k}} \succ 0.
		\end{array}
	\end{equation*}
\end{assumption}
As was done in section \ref{differential_algebraic}, the following
\begin{equation}
	\left(\begin{array}{cc}
	H_u[\hat\lambda](\wh)\\
	\\
	-\ddot{H_v}[\hat\lambda](\wh)
	\end{array}\right) = 0,
\end{equation}
along with Assumption \ref{LC-constrained} can be solved with the implicit function theorem and as a consequense, such controls are continuos in the interval $\Ih_k$. Finally, since the controls are continuous in each interval $\Ih_k$, we conclude that they satisfy for each $i = 1,\cdots, l$ and $j = 1, \cdots, m$
\begin{equation}
\label{control_bounds}
\begin{array}{c}
	-\rho < u_{min} \le \uh_i(t) \le u_{max} < 1+\rho\\
	-\rho < v_{min} \le \vh_j(t) \le v_{max} < 1+\rho 
\end{array}, \text{ on $[0,T]$}.
\end{equation}

Now, given the partition of $[0,T]$ induced by the switching times, and the arcs structure, we define the following unconstrained problem with normalized time in the interval $[0,1]$. In this new control problem the states correspond to $x^k$, the states of the original problem in the interval $I_k:=[T_{k-1}, T_k]$, where $T_k \in \mathbb{R}$ are variables of zero dynamics. Note that the latter are a rought estimate of the optimal switing times, that will be interatively tunned by the shooting algorithm. We only require $T_0 = 0$ and $T_N = T$. The controls $u^k$ and $v^k$ are defined analogously. The transformed problem (TP) in the interval $[0,1]$ is the following.
\begin{align}
	\underset{(u,v)\in \U\times\V}{\text{ minimize }} &
	\phi(x^1(0), x^N(1)) \\
	\text{subject to} & \nonumber \\
	&  \dot{x}^k(t) = (T_k - T_{k-1})f(x^k(t), u^k(t), v^k(t)), \ \ k = 1,\cdots,N\\
	&\dot{T}_k = 0, \ \ k = 1,\cdots,N\\
	&  \eta(x^1(0), x^N(T)) = 0, \ \ \\
	& x^k(1) = x^{k+1}(0), \ \ k = 1,\cdots,N-1.
\end{align}

Intuitively we obtain a solution of (TP) from (CP), and vice versa, using the following trasformation
\begin{equation*}
	\begin{array}{cc}
		\xh^k(t) &:= \xh\left(\Th_{k-1} + (\Th_k - \Th_{k-1})t\right),\\
		\uh^k(t) &:= \uh\left(\Th_{k-1} + (\Th_k - \Th_{k-1})t\right),\\
		\vh^k(t) &:= \vh\left(\Th_{k-1} + (\Th_k - \Th_{k-1})t\right),
	\end{array}
	\text{ for $t \in [0,1]$}.
\end{equation*}
Set 
\begin{equation}
	\Wh := \left(\left(\xh^k\right)_{k=1}^N, \left(\uh^k\right)_{k=1}^N, \left(\vh^k\right)_{k=1}^N, \left(\Th_k\right)_{k=1}^{N-1}\right).
\end{equation}
The relation between the solutions of (CP) and (TP) is formalized in Lemma
\begin{lemma}
	\label{CP-TP-relation}
	If $\wh$ is a Pontryagin minimum of \textnormal{(CP)}, as in definition \ref{pontryagin_minimum}, then $\Wh$ is a weak minimum of \textnormal{(TP)}.
\end{lemma}
\begin{definition}
	\label{pontryagin_minimum}
	A feasible trajectory $\wh \in \W$ is a Pontryagin minimum of problem \textnormal{(CP)} iff for any positive $N$, there exists some $\varepsilon_N > 0$ such that $\wh$ is a minimum in the set of feasible trajectories $w = (x,u,v) \in \W$ satisfying
	\begin{equation*}
		\norm{x - \xh}_{\infty} < \varepsilon_N, \ \norm{(u,v) - (\uh,\vh)}_{1} < \varepsilon_N, \ \norm{(u,v) - (\uh,\vh)}_{\infty} < N.
	\end{equation*}
\end{definition}

The strategy of our proof will be to extract the weak optimality for a solution of (TP) from the optimality of (CP) by transforming a neighborhood of optimality in the Pontryagin sense for the nominal trajectory $\wh$ into a neighborhood in the weak sense for the trajectory $\Wh$.

\begin{proof}{\em of Lemma \ref{CP-TP-relation}}
	Since we assume $\wh$ to be a Pontryagin minimum of (CP), from Definition \ref{pontryagin_minimum}, there exists $\varepsilon > 0$ such that
	\begin{equation}
		\norm{x - \xh}_{\infty} < \varepsilon, \ \norm{(u,v) - (\uh,\vh)}_{1} < \varepsilon, \ \norm{(u,v) - (\uh,\vh)}_{\infty} < 1.
	\end{equation}
	So we must find a neighborhood of $\Wh$ where it is optimal in the weak sense. In other words, we search for $\bar\delta, \bar\varepsilon > 0$, such that $\Wh$ is with respect to all feasible solutions $W = ((x^k), (u^k), (v^k), (T_k))$ that satisfy
	\begin{equation}
		\left| T_k - \Th_k\right|<\bar\delta, \ \norm{(u^k,v^k) - (\uh^k,\vh^k)}s_{\infty} < \bar\varepsilon, \ \text{ for all } k = 1, \cdots, N. 
	\end{equation}
	So for each $W$ we map into a feasible variation of (CP) 
	\begin{equation}
		\alpha(t) := \alpha^k\left(\frac{t - T_{k-1}}{T_k - T_{k-1}}\right),
	\end{equation}
	with $\alpha \in \{x,u,v\}$. Therefore, we have that $x(0) = x^1(0)$ and $x(T) = x^N(1)$ and from the feasibility of $W$, the end point constraints in \eqref{initial-final.constraints} are satisfied.
	
	The control constraints can be verified using the picewise continuity of each component of the controls, and by construction the continuity of $\left((u^k), (v^k)\right)$ in the interval $(0,1)$. Therefore, we can use equation \eqref{control_bounds} and we can choose $\bar\varepsilon$ so that
	\begin{equation}
	\begin{array}{c}
	-\rho < u_{min} - \bar\varepsilon \le u_i(t) \le u_{max} + \bar\varepsilon < 1+\rho\\
	-\rho < v_{min} - \bar\varepsilon\le v_j(t) \le v_{max} + \bar\varepsilon < 1+\rho
	\end{array}, \text{ on $[0,T]$}.
	\end{equation}
	
	In the sequence, we relate the size neighborhood around $\Th_k$ with $\varepsilon$ by finding bounds to $\norm{(u,v) - (\uh,\vh)}_{1}$. The analysis is analogous for both controls $u$ and $v$, hence we will conduct the calculations component wise only for $u$. We compute 
	\begin{equation}
		\begin{array}{cc}
			\disp \int_{I_k\cap \Ih_k} |u_i(t) - \uh_i(t)|\dd t & \disp \le
			\int_{I_k\cap \Ih_k} \left| u_i^k\left(\frac{t - T_{k-1}}{T_k - T_{k-1}}\right) - \uh_i^k\left(\frac{t - T_{k-1}}{T_k - T_{k-1}}\right) \uh_i(t)\right|\dd t \\
			& \disp + \int_{I_k\cap \Ih_k} \left| \uh_i^k\left(\frac{t - T_{k-1}}{T_k - T_{k-1}}\right) - \uh_i^k\left(\frac{t - \Th_{k-1}}{\Th_k - \Th_{k-1}}\right) \right|\dd t
		\end{array}
	\end{equation}  
	The first integral is bounded by $\varepsilon|I_k\cap \Ih_k|$ by the previous arguments. For the second term, since $\uh$ is uniformly continuous in $I_k$ and $\Ih_k$, we can find some $\bar\delta_k > |T_k - \Th_k|$ so that 
	\begin{equation*}
		\left| \uh_i^k\left(\frac{t - T_{k-1}}{T_k - T_{k-1}}\right) - \uh_i^k\left(\frac{t - \Th_{k-1}}{\Th_k - \Th_{k-1}}\right) \uh_i(t)\right| < \bar\varepsilon
	\end{equation*}
	for each $k = 1, \cdots, N$. Hence we need only choose $\bar\delta$ to be the smaller. 
	Next, we need to evaluate the integral outside this intersection. We assume w.l.o.g. that $T_k < \Th_k$ hence
	\begin{equation*}
		\int_{T_k}^{\Th_k}|u_i(t) - \uh_i(t)|\dd t \le \bar\delta\bar\varepsilon.
	\end{equation*}
	Summing all the terms, we have that $\norm{u_i - \uh_i}_1 < \varepsilon(2T + (N-1)\bar\delta)$. Thus, taking in acount all the control compenents,  $m$ from the linear controls and $l$ from the nonlinear controls, if 
	\begin{equation*}
		\bar\varepsilon(2T + (N-1)\bar\delta) < \frac{\varepsilon}{m + l},
	\end{equation*}
	then $\norm{u - \uh} < \varepsilon$, as we wished.
\end{proof}

\subsection{Pertubation of the Constrained Problem}

Consider the following control problem
\begin{equation}
\label{epsilon_CP}
\tag{\epsilon CP}
	\begin{array}{cl}
		\text{ minimize } &
		\phi(\xh(0),x(T)) \\
		\text{subject to} & \\
		& \dot{x}(t) = f(x(t), u(t), v(t)), \ \ \text{a.e. on $[0,T]$}\\
		&  \eta_j(x(0),x(T)) = 0, \ \ \text{for}  j = 1,\cdots, d_{\eta},\\
		& (u, v) \in \U_{ad}^{\epsilon} \times \V_{ad}^{\epsilon}\\
		& \U_{ad}^{\epsilon} := L^{\infty}([0,T]; U + \epsilon B(0;1)),\\
		& \V_{ad}^{\epsilon} := L^{\infty}([0,T]; V + \epsilon B(0;1)).
	\end{array}
\end{equation}

Call the optimal value of \eqref{epsilon_CP} as $V(\epsilon)$, then one notes that $V(0)$ refers to the optimal value of the original constrained problem (CP). 

We claim that the function $V:\mathbb{R} \to \mathbb{R}$ satisfies
\begin{equation}
V(0) < V(\epsilon) + \epsilon L_{\phi}e^{TL_f},
\end{equation}
and hence is l.s.c, where $L_{\phi}$ and $L_f$ are the Lipschitz coeficients of the data functions $f$ and $\phi$.

\begin{proof}
	Clearly, we have
	\begin{equation*}
	\U_{ad} \times \V_{ad} = \U_{ad}^{0} \times \V_{ad}^{0} \subset \U_{ad}^{\epsilon} \times \V_{ad}^{\epsilon},
	\end{equation*}
	hence, minimizing w.r.t. the controls $u,v$, implies that $V(\epsilon) \le V(0)$. 
	Then, for each pair $(u,v) \in \U_{ad} \times \V_{ad}$, consider an $\epsilon$-pertubation, some pair  $(u^{\epsilon}, v^{\epsilon}) \in \U_{ad}^{\epsilon} \times \V_{ad}^{\epsilon}$ such that $\norm{(u,v) - (u^{\epsilon}, v^{\epsilon})}_{\infty} < \epsilon$. 
	
	Denote by $x^{\epsilon}$ the function obtained by integrating the system with such controls and $\delta x:= x - x^{\epsilon}$. Then one has
	\begin{align*}
	|\delta \dot{x}| &= \left|f(x, u, v) - f\left(x^{\epsilon}, u^{\epsilon}, v^{\epsilon}\right)\right|\\
	&\le L_f\left(|\delta x| + |(u - u^{\epsilon}, v - v^{\epsilon})\right|.
	\end{align*} 
	With Gronwall's lemma we conclude that
	\begin{equation*}
	|\delta x(t)| \le \epsilon e^{tL_f}.
	\end{equation*}
	From the Lipschitz continuity of $\phi$ we obtain
	\begin{equation*}
	\phi(\xh(0), x(T)) \le \phi(\xh(0), x^{\epsilon}(T)) +\epsilon L_{\phi}e^{TL_f}.
	\end{equation*}
	However, since we choose an arbitrary $\epsilon$-perturbation of the controls, we can obtain any element in $\U_{ad}^{\epsilon} \times \V_{ad}^{\epsilon}$ choosing apropriate $(u,v) \in \U \times \V$ and afterwards a fitting variation, that can also be null. Therefore, minimization in $ \U \times \V$ we get
	\begin{align*}
	V(0) & \le  V(\epsilon) + \epsilon L_{\phi}e^{TL_f}.
	\end{align*}
\end{proof}

==> delta_sing.tex <==

\begin{equation}
	\sloppy
	p_{\gamma} \left(- \left(\frac{p_{\gamma}^{3}}{m p_{v}^{3} v^{5} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{2 p_{\gamma}}{m p_{v} v^{3} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) \left(\frac{p_{\gamma} \cos{\left (\gamma \right )}}{m p_{v} r^{2} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{6200 v^{2}}{m^{2}} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500} + \frac{6200 v e^{- 500 r + 500}}{m^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right)\right) + \left(- \frac{p_{\gamma}}{p_{v} v^{2} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)} \left(\frac{p_{\gamma}^{4}}{m p_{v}^{4} v^{4} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{p_{\gamma}^{2}}{m p_{v}^{2} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{p_{\gamma}^{2}}{m p_{v}^{2} v^{2} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} + \frac{1}{m \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) + \frac{p_{\gamma}}{p_{v}^{2} v \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)} \left(\frac{p_{\gamma}^{4}}{m p_{v}^{3} v^{5} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{2 p_{\gamma}^{2}}{m p_{v} v^{3} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{p_{\gamma}^{2}}{m p_{v} v^{3} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}}\right)\right) \left(\frac{p_{\gamma}}{m p_{v} v \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\left(\frac{1}{r} + \frac{1}{r^{2} v^{2}}\right) \cos{\left (\gamma \right )} + \frac{542.5 p_{\gamma}}{m p_{v} v} e^{- 500 r + 500}\right) + \frac{\left(\frac{v}{r} - \frac{1}{r^{2} v}\right) \sin{\left (\gamma \right )}}{m v \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} - \frac{1}{m v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(- \frac{1}{r^{2}} \sin{\left (\gamma \right )} - \frac{3100 v^{2}}{m} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500}\right)\right) + \frac{p_{\gamma}}{m p_{v} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\frac{p_{\gamma} \left(\frac{v}{r} - \frac{1}{r^{2} v}\right) \cos{\left (\gamma \right )}}{m p_{v} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{p_{\gamma} \cos{\left (\gamma \right )}}{m p_{v} r^{2} v^{3} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{\left(\frac{1}{r} + \frac{1}{r^{2} v^{2}}\right) \sin{\left (\gamma \right )}}{m \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) + \frac{1}{m \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\frac{p_{\gamma}^{3} \left(\frac{v}{r} - \frac{1}{r^{2} v}\right) \sin{\left (\gamma \right )}}{m p_{v}^{3} v^{5} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{p_{\gamma}^{3}}{m p_{v}^{3} v^{6} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} \left(- \frac{1}{r^{2}} \sin{\left (\gamma \right )} - \frac{3100 v^{2}}{m} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500}\right) - \frac{p_{\gamma}^{2}}{m p_{v}^{2} v^{3} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} \left(\left(\frac{1}{r} + \frac{1}{r^{2} v^{2}}\right) \cos{\left (\gamma \right )} + \frac{542.5 p_{\gamma}}{m p_{v} v} e^{- 500 r + 500}\right) + \frac{p_{\gamma} \left(\frac{1}{r} + \frac{1}{r^{2} v^{2}}\right) \sin{\left (\gamma \right )}}{m p_{v} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} - \frac{2 p_{\gamma} \left(\frac{v}{r} - \frac{1}{r^{2} v}\right) \sin{\left (\gamma \right )}}{m p_{v} v^{3} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} - \frac{p_{\gamma}}{m p_{v} v^{3} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\frac{271.25 p_{\gamma}^{2}}{m p_{v}^{2} v} e^{- 500 r + 500} - \frac{6200 v}{m} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500}\right) + \frac{3 p_{\gamma}}{m p_{v} v^{4} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(- \frac{1}{r^{2}} \sin{\left (\gamma \right )} - \frac{3100 v^{2}}{m} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500}\right) - \frac{1}{m \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(- \frac{2}{r^{2} v^{3}} \cos{\left (\gamma \right )} - \frac{542.5 p_{\gamma}}{m p_{v} v^{2}} e^{- 500 r + 500}\right)\right) + \frac{2 p_{\gamma} \left(\frac{v}{r} - \frac{1}{r^{2} v}\right) \sin{\left (\gamma \right )}}{m^{2} p_{v} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} - \frac{2 p_{\gamma}}{m^{2} p_{v} v^{3} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(- \frac{1}{r^{2}} \sin{\left (\gamma \right )} - \frac{3100 v^{2}}{m} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500}\right) - \frac{2}{m^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\left(\frac{1}{r} + \frac{1}{r^{2} v^{2}}\right) \cos{\left (\gamma \right )} + \frac{542.5 p_{\gamma}}{m p_{v} v} e^{- 500 r + 500}\right) - \frac{4340.0 p_{\gamma}}{m^{3} p_{v}} e^{- 500 r + 500} + \frac{6200 p_{\gamma} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500}}{m^{3} p_{v} v \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} - \frac{1085.0 p_{\gamma} e^{- 500 r + 500}}{m^{3} p_{v} v \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) + p_{r} \left(\left(- \frac{p_{\gamma}}{p_{v} v^{2} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)} \left(\frac{p_{\gamma}^{4}}{m p_{v}^{4} v^{4} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{p_{\gamma}^{2}}{m p_{v}^{2} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{p_{\gamma}^{2}}{m p_{v}^{2} v^{2} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} + \frac{1}{m \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) + \frac{p_{\gamma}}{p_{v}^{2} v \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)} \left(\frac{p_{\gamma}^{4}}{m p_{v}^{3} v^{5} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{2 p_{\gamma}^{2}}{m p_{v} v^{3} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{p_{\gamma}^{2}}{m p_{v} v^{3} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}}\right)\right) \left(\frac{p_{\gamma} \sin{\left (\gamma \right )}}{m p_{v} v \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} - \frac{\cos{\left (\gamma \right )}}{m \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) + \frac{p_{\gamma}}{m p_{v} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\frac{p_{\gamma} \sin{\left (\gamma \right )}}{m p_{v} v \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} - \frac{\cos{\left (\gamma \right )}}{m \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) + \frac{1}{m \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(- \frac{p_{\gamma}^{3} \cos{\left (\gamma \right )}}{m p_{v}^{3} v^{4} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{p_{\gamma}^{2} \sin{\left (\gamma \right )}}{m p_{v}^{2} v^{3} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} + \frac{p_{\gamma} \cos{\left (\gamma \right )}}{m p_{v} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) - \frac{2 p_{\gamma} \cos{\left (\gamma \right )}}{m^{2} p_{v} v \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} - \frac{2 \sin{\left (\gamma \right )}}{m^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) + p_{v} \left(\left(\frac{\cos{\left (\gamma \right )}}{m r^{2} v \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} - \frac{6200 p_{\gamma} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500}}{m^{2} p_{v} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) \left(- \frac{p_{\gamma}}{p_{v} v^{2} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)} \left(\frac{p_{\gamma}^{4}}{m p_{v}^{4} v^{4} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{p_{\gamma}^{2}}{m p_{v}^{2} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{p_{\gamma}^{2}}{m p_{v}^{2} v^{2} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} + \frac{1}{m \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}}\right) + \frac{p_{\gamma}}{p_{v}^{2} v \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)} \left(\frac{p_{\gamma}^{4}}{m p_{v}^{3} v^{5} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{2 p_{\gamma}^{2}}{m p_{v} v^{3} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{p_{\gamma}^{2}}{m p_{v} v^{3} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}}\right)\right) - \frac{p_{\gamma}^{2}}{m p_{v}^{2} v^{3} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} \left(\frac{p_{\gamma} \cos{\left (\gamma \right )}}{m p_{v} r^{2} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{6200 v^{2}}{m^{2}} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500} + \frac{6200 v e^{- 500 r + 500}}{m^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right)\right) + \frac{1}{m \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\frac{p_{\gamma}^{3} \cos{\left (\gamma \right )}}{m p_{v}^{3} r^{2} v^{5} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{2 p_{\gamma} \cos{\left (\gamma \right )}}{m p_{v} r^{2} v^{3} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} - \frac{542.5 p_{\gamma}^{2}}{m^{2} p_{v}^{2} v} e^{- 500 r + 500} + \frac{6200 p_{\gamma}^{2} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500}}{m^{2} p_{v}^{2} v^{2} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)^{\frac{3}{2}}} - \frac{542.5 p_{\gamma}^{2} e^{- 500 r + 500}}{m^{2} p_{v}^{2} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{12400 v}{m^{2}} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500} + \frac{6200 e^{- 500 r + 500}}{m^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right)\right) - \frac{p_{\gamma}^{2} \sin{\left (\gamma \right )}}{m^{2} p_{v}^{2} r^{2} v^{4} \left(\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1\right)} + \frac{2 p_{\gamma} \cos{\left (\gamma \right )}}{m^{2} p_{v} r^{2} v^{2} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} + \frac{24800 v^{2}}{m^{3}} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right) e^{- 500 r + 500} + \frac{24800 v e^{- 500 r + 500}}{m^{3} \sqrt{\frac{p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 1}} \left(\frac{0.04375 p_{\gamma}^{2}}{p_{v}^{2} v^{2}} + 0.05\right)\right)
\end{equation}

==> diff_alg_backup.tex <==
The {\em Pontryagin Maximum Principle} implies that the local solution of the optimization problem \eqref{unconstrained.problem} in a function space is the solution of a {\em two-point boundary value problem} (TPBVP), provided that we are able to write the controls as a function of the state and costates. Such (TPBVP) consists in the original dynamics of the states and the new introduced dynamics of the costates, with the algebraic constraints given by the  initial-final constraints, transversality and stationarity conditions.

In this paper, we propose an algorithm to numerically solve this {\em differential-algebraic} system. The first step is to find a suitable representation of the controls as a smooth function of the states and costates.

In the following discussion we shall present a strategy to achieve this substitution of the controls that is a combination of the techniques in the particular cases when all the controls appear nonlinearly in the dynamics (this is for $m = 0$) and when the controls are totally {\em affine} (i.e. when $l = 0$). Next we give a brief review for each of these simpler cases and finally propose a technique for our mixed case.

However, we can trace a systematic approach that is common to all cases. It consists in using the stationarity of the Hamiltonian or any immediate consequence of in conjunction to a set of necessary conditions usually known as Legendre-Clesbch conditions to write a system of the form
\begin{equation}
\tag{IFTsys}
\label{IFTsys}
	\begin{array}{rc}
	\Theta(\xi, \alpha) &= 0\\
	D_{\alpha}\Theta(\xi, \alpha) &\succ 0
	\end{array}.
\end{equation} 

The {\em Implicit Function Theorem}


\subsection{The totally nonlinear case} When we have no affine controls in the dynamics, the classical approach is to use the stationarity of the Hamiltonian to write the control as a function of the states and costates.
\begin{equation}
	\label{representation.nonlin}
	\uh(t) = U(\xh(t), \ph(t))
\end{equation}

Using the stationarity of the Hamiltonian \eqref{stationarity.Hamiltonian} and the {\em Implicit Function Theorem (IFT)}, one can achieve \eqref{representation.nonlin}. However, to satisfy the requirements of the {\em (IFT)}, the following assumption is necessary.
\begin{assumption}[Strengthened Legendre-Clebsch condition]
	\label{strengthenedLC}
	The second derivative of the Hamiltonian function, with respect to the control is positive definite,
	\begin{equation*}
		H_{uu}[ \lambda](\wh) \succ 0.
	\end{equation*}
\end{assumption}
In fact, the second partial derivative of the Hamiltonian function with respect to the control being positive semi-definite is a necessary condition for optimality of a trajectory, therefore, this assumption is a not too strong. In the future we shall show that this necessary condition holds if one assumes the uniqueness of the Lagrange multipliers, that is a consequence of Assumption \ref{qualification.constraints}. 

\subsection{The totally affine case} When the controls appear linearly, we immediately face complications concerning the Strengthened Legendre-Clesbch condition, since the affine nature of the controls implies that the matrix $H_{vv}$ is null. Therefore, the process for achieving a representation for the optimal control in terms of the states as
\begin{equation}
	\label{representation.linear}
	\vh(t) = V(\xh(t), \ph(t))
\end{equation}
is not so trivial.

The solution for such problem is to turn our analysis to the time derivatives of $H_v$, which is some times referred as the {\em switching function}. Following the notation in \cite{aronna2013shooting}, we define the switching function
\begin{equation}
	\label{switching.function}
	\begin{array}{rl}
		\Phi \colon [0,T] &\to \mathbb{R}^m\\
		t &\mapsto H_{v}[\lambda](\wh) = \left(\ph(t)\cdot f_i(\xh(t))\right)_{i = 1}^m. 
	\end{array}
\end{equation}

We shall try to extract the optimal control from the time derivatives of the switching function \eqref{switching.function}. To simplify our analysis, consider a vector field $F:\mathbb{R}^n \to \mathbb{R}^n$ that is a function only of the states, that is $F = F(x)$, we will evaluate the time derivative of the scalar function $\ph \cdot F(x)$
\begin{align}
	\frac{\dd}{\dd t}(\ph \cdot F(\xh)) &= \dot{\ph}\cdot F(\xh) + \ph \cdot D_x F(\xh) \dot{\xh}\\
								   &= \ph \cdot\left( D_x F(\xh)f_0(\xh) - D_x f_0(\xh)F(\xh) + \sum_{i = 1}^m \vh_i \left(  D_x F(\xh)f_i(\xh) - D_x f_i(\xh)F(\xh)\right) \right).
\end{align}

Before proceeding it is advantageous to introduce the definition of {\em Lie brackets}. Given two $\C^1$ functions $g,h$ the Lie bracket is denoted as
\begin{equation}
	\label{Lie.Brackets}
	[g,h]^x := D_x h(x)g(x) - D_x g(x)h(x).
\end{equation}

Using the new introduced notation, we can write
\begin{equation}
	\label{genericvectorfield.D1}
	\frac{\dd}{\dd t}(\ph \cdot F(x)) = \ph \cdot [f_0, F]^x + \sum_{i = 1}^m \vh_j \ph \cdot [f_i, F]^x.
\end{equation}

We can obtain the first time derivative of the component of index $i$ of the switching function by choosing $F = f_i$ so that Equation \eqref{genericvectorfield.D1} becomes
\begin{equation}
	\label{switching.function.D1_preview}
	\dot{H}_{v_j}[\hat\lambda](\wh) = \ph \cdot [f_0, f_j]^x + \sum_{i = 1}^m \vh_j \ph \cdot [f_i, f_j]^x.
\end{equation}

The difficulties arise since this derivative is independent of the control function when evaluated at the optimal trajectory. This is a consequence of the following proposition which is a corollary of second order necessary conditions for the optimality when the set of multipliers is a singleton. This is the case of our problem in virtue of Assumption \ref{qualification.constraints}. 

\begin{proposition}[Goh conditions]
	\label{Goh.condition}
	Assume that $\wh(\cdot)$ is a weak minimum having an unique multiplier. Then the following identity holds
	\begin{equation*}
		\ph \cdot [f_i, f_j]^x(\cdot) = 0, \quad \text{ for $i,j = 1, \cdots, m$}.
	\end{equation*}
\end{proposition} 

Proposition \ref{Goh.condition} was first introduced by Goh, and was further generalized by Aronna \footnote{ The credit for this result is given to Aronna and many others, check the literature for accurate references.} . The reader is referred to Corollary 5.2 of \cite{aronna2017second} for a proof. It is a direct consequence that the time derivative of the switching function \eqref{switching.function.D1_preview} can now be expressed as
\begin{equation}
	\label{switching.function.D1}
	\dot{H}_{v_i}[\hat\lambda](\wh) = \ph \cdot [f_0, f_i]^x,
\end{equation}

showing explicitly the independence on the controls. Our hope is to turn to the second time derivative, which can be achieved with equation \eqref{genericvectorfield.D1}, this time choosing $F =  [f_0, f_i]^x$. We obtain
\begin{equation}
	\label{switching.function.D2}
	\ddot{H}_{v_i}[\hat\lambda](\wh) = \ph \cdot \left[f_0,  [f_0, f_i]^x\right]^x+\sum_{j = 1}^m \vh_j \ph \cdot \left[f_j,  [f_0, f_i]^x\right]^x.
\end{equation}

\begin{remark}
	One could easily be mislead into thinking that the control shall appear explicitly in equation \eqref{switching.function.D2}, as was the case with the first derivative. In fact, as was proved by {\em Kelly et al.}\cite{kelley19673}, for each control index $i$, the order $M_i$ of the first derivative of the switching function which presents the control explicitly is even.\footnote{
		
		{\bf Future work:} Could we reproduce Kelly's results in our context and using our notation (Lie bracket)?	
		
	} 
	
	This is equivalent to for every odd integer $\nu$
	\begin{equation}
		\frac{\dd ^\nu H_{v}}{\dd t^{\nu}} [\hat\lambda](\wh) = 0
	\end{equation}
	is not explicitly dependent of the control $\vh$, and therefore, it can not be used in order to achieve a representation as in Equation \eqref{representation.linear}.
\end{remark}

The way to proceed then is to take as many derivatives as necessary in order to force the explicit appearance of the linear controls. For simplicity, we shall consider that such task is achieved with only two derivatives. From the stationarity of the Hamiltonian for the linear controls, we have $\ddot{H}_v[\lambda](\wh) = 0$. As a consequence, the controls can be retrieved by means of the {\em (IFT)}, once we assume the following {\em strengthened generalized Legendre-Clebsch conditon}.

\begin{assumption}[Strengthened Generalized Legendre-Clebsch conditon]
	\label{strengethenedLC.generalized}
	\begin{equation*}
		-\frac{\partial \ddot{H_v}}{\partial v}
		[\hat 
		\lambda](\wh) \succ 0.
	\end{equation*}
\end{assumption} 

Once again, as in the totally non linear case, the positive semi-definiteness of the quantity in Assumption \ref{strengethenedLC.generalized} is a necessary condition for the optimality of a feasible trajectory. Finally the controls can be retrieved and we substitute their expressions in the state and costate dynamics, again obtaining a two point boundary value problem. 

\subsection{The partially-affine case:}
Our strategy is to use the Implicit Function Theorem in order to obtain a representation for both $\uh$ and $\vh$ as a function of $\xh$ and $\ph$. For this, we shall make use of the stationarity of the Hamiltonian, \eqref{stationarity.Hamiltonian}, in combination with Assumptions \ref{strengthenedLC} and \ref{strengethenedLC.generalized} in order to satisfy the requirements of the theorem. 

As for the conventional Legendre-Clebsch condition, it still holds in this case, since it is a necessary condition for optimality as previously discussed. For our problem it assumes the form 
\begin{equation}
	\label{LegendreClebsch.mixed}
	\tag{LC}
	 \left(
	 \begin{array}{cc}
	 	H_{uu}[\hat\lambda](\wh) & H_{uv}[\hat\lambda](\wh)\\
	 	\\
	 	
	 	H_{vu}[\hat\lambda](\wh)
	 	 & H_{vv}[\hat\lambda](\wh)
	 \end{array}
	 \right)
	 \succeq 0.
\end{equation}
A proof of this can be found in Aronna \cite{aronna2017second}, see Corollary 1. Furthermore, since $H_{vv}[\lambda](\wh) = 0$, this condition holds if, and only if, 
\begin{equation}
	\label{LegendreClebsch.mixed.equivalent}
	H_{uu}[\lambda](\wh) \succeq 0 \text{ and } H_{uv}[\lambda](\wh) = 0.
\end{equation}

In order to find the representation analogous to \eqref{representation.nonlin} and \eqref{representation.linear}, we proceed in a similar manner. The stationarity condition for the nonlinear controls $H_u[\lambda](\wh) = 0$ can be differentiated assuming temporary enough regularity, giving
\begin{equation}
	\dot{H}_u[\lambda](\wh) = H_{ux}[\lambda](\wh) \dot{\xh} + H_{up}[\lambda](\wh) \dot{\ph} + H_{uu}[\lambda](\wh) \dot{\uh} + H_{uv}[\lambda](\wh) \dot{\vh} = 0.
\end{equation}

To formalize such expression, we make the following assumption on the controls.
\begin{assumption}[Regularity of the controls]
	\label{regularity.controls}
	The nonlinear control $\uh(\cdot)$ is continuously differentiable and the linear control $\vh(\cdot)$ is continuous. 
\end{assumption}

Note that in fact we only need them to be in the Sobolev space $W^{1,\infty}$, however it is also a requirement for proving the convergence of the shooting algorithm proposed further on.

The coefficient referent to $\dot{v}$ vanishes in virtue of \eqref{LegendreClebsch.mixed.equivalent}. We can lose the dependence of the derivative of the nonlinear controls, for this define the function $F(\xh, \uh, \vh, \ph, \dot{\uh}) = \dot{H}_u[\lambda](\wh)$. Using the last equation and assuming the strengthened Legendre-Clebsch condition we write the system
\begin{align}
	F(\xh, \uh, \vh, \ph, \dot{\uh}) &= 0\\
	D_{\dot{\uh}} F(\xh, \uh, \vh, \ph, \dot{\uh}) &\succ 0.
\end{align}
This enables us to apply the Implicit Function Theorem, giving the derivative of the nonlinear controls in the form
\begin{equation}
	\label{representation.nonlin.derivative}
	\dot{\uh}(t) = \Gamma^u(\uh, \vh, \xh, \ph),
\end{equation}
where $\Gamma$ is a $\C^1$ function, as a consequence of the $(IFT)$ as well.

Using Equation \eqref{switching.function.D1}, in our new setting we obtain
\begin{equation}
	\dot{H}_{v_i} = \ph \cdot [f_0, f_i]^x + \dot{H}_{v_iu}\dot{\uh}.
\end{equation}
We can therefore use the representation for $\dot{\uh}(\cdot)$ and differentiate one more time, obtaining
\begin{equation}
	\ddot{H}_{v_i} = \ph \cdot \left[f_0,  [f_0, f_i]^x\right]^x+\sum_{j = 0}^m \vh_j \ph \cdot \left[f_j,  [f_0, f_i]^x\right]^x + \frac{\dd }{\dd t}\left( H_{v_iu}\Gamma_u \right).
\end{equation} 
Therefore, $\ddot{H}_{v} = \ddot{H}_{v}(\wh, \ph, \dot{\vh})$, since any dependence on the time derivative of the nonlinear controls can be substituted by the representation \eqref{representation.nonlin.derivative}. In a similar manner as for the nonlinear controls, if we choose the function $F = -\ddot{H}_{v}$, then the stationarity conditions and the strengthened generalized Legendre-Clebsch condition gives the system  
\begin{align}
	F(\xh, \uh, \vh, \ph, \dot{\vh}) &= 0\\
	D_{\dot{v}} F(\xh, \uh, \vh, \ph, \dot{\vh}) &\succ 0.
\end{align}
This once again satisfies the Implicit Function Theorem and gives the representation
\begin{equation}
	\label{representation.lin.derivative}
	\dot{\vh}(t) = \Gamma^v(\uh, \vh, \xh, \ph).
\end{equation}

This finally shows that $\ddot{H}_{v}$ is a function of the states, costates and controls only and we turn to the mapping
\begin{equation}
	(w, \lambda) \mapsto
	\left(\begin{array}{cc}
		H_u[\hat\lambda](\wh)\\
		\\
		-\ddot{H_v}[\hat\lambda](\wh)
	\end{array}\right)
\end{equation}
that has derivate with respect to the controls at $(\wh, \hat \lambda)$ given by
\begin{equation}
	\J :=
	\left(\begin{array}{cc}
		\disp
		H_{uu}[\hat \lambda](\wh) & H_{uv}[\hat \lambda](\wh) \\
		& \\
		\disp
		-\frac{\partial \ddot{H}_v[\hat \lambda](\wh)}{\partial u} &\disp  -\frac{\partial \ddot{H}_v[\hat \lambda](\wh)}{\partial v}
	\end{array}\right).
\end{equation}

Since \eqref{LegendreClebsch.mixed} holds along the optimal trajectory and in virtue of the strengthened Legendre Clebsch conditions holds, assumptions \ref{strengthenedLC} and \ref{strengethenedLC.generalized}, the matrix $\J$ is positive definite and we can once again use the Implicit Function Theorem to write the desired representations as in \eqref{representation.nonlin} and \eqref{representation.linear}. This is summarized in the following proposition.

\begin{proposition}[Elimination of the controls]
	\label{control.elimination}
	If $\wh$ is a weak solution for problem \eqref{unconstrained.problem} with a single multiplier, provided that assumptions \ref{regularity.controls}, \ref{strengthenedLC} and \ref{strengethenedLC.generalized} are satisfied, then one has the representation
	\begin{equation}
	\label{control.elimination.equation}
		\uh = \Uh(\xh, \ph) \quad \vh = \Vh(\xh, \ph),
	\end{equation}
	where $U$ and $V$ are smooth function of the states and costates.
\end{proposition}

The previous discussion enable us to write the optimal control problem at hand as a two point boundary value problem as in the previous cases. Taking in account the initial-final constraints and the stationarity of the Hamiltonian as well, we obtain an equivalent differential-algebraic system of equations formed from \eqref{unconstrained.problem}, \eqref{costate_dynamics}, \eqref{transversality.conditions} and \eqref{stationarity.Hamiltonian}. Such problem, also called the {\em Optimality System}, is written as
\begin{equation}
	\label{optimality.system}
	\tag{OS}
	\left\{\begin{array}{l}
		\disp
		\dot{x} = f(x,U(x,p), V(x,p)), \text{ a.e. on $[0,T],$}\\
		\\
		\disp
		\dot{p} = -p\cdot D_xf(x,U(x,p), V(x,p)), \text{ a.e. on $[0,T],$}\\
		\\
		\eta_j(x_0, x_T) = 0 \text{ for } j = 1, \cdots, d_{\eta},\\
		\\
		p(0) = -D_{x_0}l[\lambda](x(0), x(T)),\\
		\\
		p(T) = D_{x_T}l[\lambda](x(0), x(T)),\\
		\\
		H_v(x(T), U(x(T), p(T))) = 0,\\
		\\
		\dot{H}_v(x(0), U(x(0), p(0))) = 0.\\
	\end{array}\right.
\end{equation}

We note that the first and second equations in \eqref{optimality.system} represent the state and costate dynamics, the third, the initial-final restrictions in problem \eqref{unconstrained.problem}. The transversality conditions \eqref{transversality.conditions} are represented in the forth and fifth equations. Finally, the stationarity of the Hamiltonian are implicitly satisfied by the substitution of the controls from Proposition \ref{control.elimination}, since such substitutions are equivalent to $H_u[\hat\lambda](\wh) = 0$ and $\ddot{H}_v[\lambda](\wh) = 0$. The stationarity with respect to the linear controls is retrieved with the last two equations from \eqref{optimality.system}.
	

==> gaussnewton.tex <==

In this appendix we further discuss the formulation and convergence properties of the Gauss-Newton method. Even thought we have chosen a notation that is consistent with our purposes of finding the roots of the Shooting function, the analysis here is applicable to any problem were the Gauss-Newton method is suitable. For simplicity we allow the abuse of notation that $\cals : \mathbb{R}^n \to \mathbb{R}^m$. The reader is advised not to mistake $n$ and $m$ with the dimensions of the states and nonlinear controls.

We remind that our primal objective is to solve
\begin{equation}
\label{shooting.function.reminder}
	\cals (\hat \nu) = 0.
\end{equation} 

Such problem is equivalent to solving the optimization problem
\begin{equation}
\label{equivalent.optimization.problem}
	\min_{\nu \in D(\cals)} \left|\cals(\nu)\right|^2.
\end{equation}  

In the order hand, first order conditions of optimality for this convex problem make \eqref{shooting.function.reminder} and \eqref{equivalent.optimization.problem} equivalent. In turn we make updates in the approximations of the solutions as $ \nu_{k+1} = \nu_{k} + \Delta_k$ where $\Delta_k$ is the solution of the least squares problem 
\begin{equation}
\label{linear.approximation}
		\disp \min_{\Delta \in D(\cals)} \left|\cals(\nu_k) + \cals'(\nu_k)\Delta\right|^2.
\end{equation}
That is an interactive approach to solve \eqref{equivalent.optimization.problem} done by means of a first order Taylor expansion, finding consecutive linear approximations. 

While $\Delta_k$ can be expressed as the solution of
\begin{equation}
	\label{gonnausethis}
	S'(\nu_k)^TS'(\nu_k) \Delta_k + S'(\nu_k)^TS(\nu_k) = 0,
\end{equation} 
and explicitly written provided that $S'(\nu_k)^TS'(\nu_k)$ is invertible, we shall still have some error at each approximation that comes from the truncation of the residual terms from the Taylor expansion. Since there are various estimates of such error depending on the regularity of the objective function, we can also have different speeds of convergence depending on such regularity. This discussion is formalized in the following theorem. 

\begin{theorem}[Gauss-Newton convergence]
	\label{GaussNewton.convergence}
	Let $\hat\nu$ be a solution of problem \eqref{shooting.function.reminder}, such that the matrix $	S'(\hat\nu)^TS'(\hat\nu)$ is nonsingular. Consider also the sequence $(\nu_k)_{k \in \mathbb{N}}$ defined as in \eqref{linear.approximation} and such that $\nu_0$ is chosen sufficiently close to the solution so that $	S'(\nu_0)^TS'(\nu_0)$ is still non singular at this point. Then the Gauss Newton method converges at least linearly. Moreover, in case the function $S'(\cdot):\mathbb{R}^n\to\mathbb{R}^{m\times n}$ is Lipschitz continuous, quadratic convergence holds. 
\end{theorem}
\begin{proof}
	We define $\epsilon_k := \nu_k - \hat\nu$, the error of each approximation of the solution using the Gauss Newton method. Consider the following first order Taylor expansion of the objective function
	\begin{equation}
		\label{shooting.function.1storderTalor}
		S(\nu_k + h) = S(\nu_k) + S'(\nu_k)\cdot h + r(h),
	\end{equation}
	where $r$ is the residual of the Taylor expansion. 
	We chose $h = -\epsilon_k$ so that the left side of \eqref{shooting.function.1storderTalor} vanishes, since it is evaluated at the solution. We obtain
	\begin{equation}
		\label{GNtheocheck1}
		S(\nu_k) - S'(\nu_k)\cdot \epsilon_k + r(-\epsilon_k) = 0.
	\end{equation}
	Multiplying both sides by $S'(\nu_k)^T$ and using the definition of $\Delta_k$ in \eqref{gonnausethis}, we can write
	\begin{equation}
	\label{GNtheocheck2}
	  \epsilon_k + \Delta_k = \left(S'(\nu_k)^TS'(\nu_k)\right)^{-1}r(-\epsilon_k),
	\end{equation}
	since we assumed the sequence to be close enough to $\hat\nu$ so that, for each element of the sequence, the inverse is well defined and bounded. We call the reader's attention to the fact that $\epsilon_k + \Delta_k = \epsilon_{k+1}$ and turn to the analysis of the term $r(\epsilon_k)$. If we consider the derivative $ S'(\cdot)$ to be Lipschitz continuous, then the second order derivative is  defined almost everywhere and the residual can be written as 
	\begin{equation}
	\label{residual.integral}
		r(\epsilon_k) = \int_0^1 S'(\nu_k + t\epsilon_k)\cdot \epsilon_k \dd t. 
	\end{equation}  
	Since $S'(\cdot)$ is continuous in the neighborhood of interest, the sequence $(S'(\nu_k))_{k \in \mathbb{N}}$ is bounded. Also note that
	\begin{equation}
		 0 = S(\hat \nu) = \int_0^1 S'(\hat \nu + t(\nu_k -\hat \nu)) \cdot \epsilon_k \dd t,
	\end{equation}
	and summing this integral to \eqref{residual.integral}, one obtains
	\begin{equation}
		|r(\epsilon_k)| \le \left| \int_0^1 \left( S'(\nu_k + t\epsilon_k) - S'(\hat \nu + t\epsilon_k))\right) \dd t \right||\epsilon_k| = \cO\left(|\epsilon_k|^2\right).
	\end{equation}
	The last equality is valid given that $S'(\cdot)$ is Lipschitz. Therefore, we have $|\epsilon_{k+1}| = \cO\left(|\epsilon_{k}|^2\right)$ and there exists some constant $c>0$ that satisfies the estimate
	\begin{equation}
		\label{GN.quadratic.estimate}
		|\epsilon_{k+1}| \le c|\epsilon_{k}|^2.
	\end{equation}
	If the initial approximation is chosen close enough so that $|\epsilon_0| = |\nu_0 - \hat\nu|<\frac{\varepsilon}{c}$, where $0 < \varepsilon < 1$, then we can easily show with finite induction that 
	\begin{equation}
		|\epsilon_k| \le \frac{\varepsilon^{2k}}{c},
	\end{equation}
	proving that the sequence $(\nu_k)_{k \in \mathbb{N}}$ converges quadratically to $\hat\nu$.
	
	When we drop the assumption on $S'(\cdot)$ begin Lipschitz continuous, through the same analysis of the Taylor expansion of the objective function, the residual is of the form $r(|\epsilon_k|) = o(|\epsilon_k|)$ and we write
	\begin{equation}
		\label{GN.estimate.smallo}
		|\epsilon_{k+1}| = |\epsilon_k|\rho(|\epsilon_k|),
	\end{equation}
	where the function $\rho(|\epsilon_k|)$ approaches zero whenever $|\epsilon_k|\rightarrow 0$. So, given some $0<\varepsilon<1$, there exists some $\delta > 0$ such that when $|\epsilon_0|<\delta$, we have that $|\epsilon_1| < \varepsilon |\epsilon_0|$. 
	
	Proceeding inductively, we check that $|\epsilon_k| < \varepsilon |\epsilon_{k-1}|$, since $\varepsilon < 1$, and our induction hypothesis holds $|\epsilon_k| < |\epsilon_0| < \delta$, implying that $\rho(|\epsilon_k|) < \epsilon$. With \eqref{GN.estimate.smallo}, this gives the estimate
	\begin{equation}
	\label{GN.linear.estimate}
		|\epsilon_{k}| < \varepsilon^k |\epsilon_0|,
	\end{equation}
	proving the linear convergence.
\end{proof}

In the text the assumptions of this theorem, for the convergence of the Gauss-Newton method are implied since the derivative of the shooting function is one-to-one. This implies that 
\begin{equation*}
S'(\nu_k)^TS'(\nu_k)\nub = 0
\end{equation*}
if, and only if, $\nub$ is the null vector and hence $S'(\nu_k)^TS'(\nu_k)$ is nonsingular. 
	
	
	

==> obtaining_linear_controls.tex <==
{\color{red} NEW DRAFT}\\ 

As discussed in section \ref{differential_algebraic}, we still lack a expression to the linear controls from which we can extract numerical values. This can be done as before, assembling linear systems from equation \eqref{control.elimination.equation}. Since the problem (TP) is unconstrained, we can just use the linear system given in equations \eqref{lin_cont.lin_sys,kernel_equation}. However, for the sake of economy of computations and notation, given some candidate solution $W$, we use tranformation \eqref{transform.CP-TP}. 

Note that, at time $t \in I_k$, for $i \in S_k$ Pontryagin's Maximum Principle still implies that $\ddot{H}_{v_i} = 0$. Hence equation \eqref{control.elimination.equation} holds and using the transformation \eqref{transform.TP-CP.xu}\eqref{transform.TP-CP.v}, for $i \in S_k$ we have
\begin{equation}
\label{kernel_equation.prev.k}
\begin{array}{rl}
0 &= \disp  \sum_{j\in S_k}v^k_jp^k\cdot\left(  \left[f_j^k,\left[f_0^k,f_i^k\right]^x\right]^x + \left[U^k, p^k\cdot f^k_i\right]^{x,p}\right) +\\
  & \disp \sum_{j \in B_k \cup \{0\}}p^k\cdot\left( \left[f_j^k,\left[f_0^k,f_i^k\right]^x\right]^x + \left[U^k, p^k\cdot f^k_i\right]^{x,p}\right).
\end{array}
\end{equation}
The superscript $k$ denotes that the quantitie was evaluated at $W$, {\em e.g.} $f_i^k = f_i\left(x^k, u^k\right)$.

Defining the quantities, for each $k = 1, \dots, N$ and for each time $t \in [0,1]$
\begin{equation}
\label{lin_cont.lin_sys.k}
\begin{array}{c}
\disp \Gamma^k = \left(\gamma_{ij}^k \right)_{\tiny
	\begin{array}{c}
	i = 1,\dots,m\\
	j = 0,\dots,m
	\end{array}
}
\disp \gamma_{ij}^k = p^k\cdot\left(  \left[f_j^k,\left[f_0^k,f_i^k\right]^x\right]^x + \left[U^k, p^k\cdot f^k_i\right]^{x,p}\right).
\end{array}
\end{equation}
Then obtaining the optimal linear controls $v^k(t)$, at time $t \in [0,1]$, reduces to solving the convex optimization problem
\begin{equation}
	\label{obtain_lin_cont}
	\begin{array}{cl}
		\underset{\vt \in \mathbb{R}^{m+1}}{\text{minimize}}& \norm{\Gamma^k\vt}_2^2 \\
		\text{subject to: }& 
		\left(
		\begin{array}{c}
			\left(\mathds{1}_{1\times j}\right)_{j \in \{0\}\cup B_k}\\
			\left(\mathds{1}_{1\times j}\right)_{j \in A_k}
		\end{array}
		\right)\vt = 
		\left(
		\begin{array}{c}
			\mathds{1}_{1+|B_k|\times 1}\\
			0_{|A_k|\times 1}
		\end{array}
		\right)\\
	& \left( 
	\begin{array}{c}
		I_{S_k}\\
		-I_{S_k}
	\end{array}
	\right) \le 
	\left(
	\begin{array}{c}
		\mathds{1}_{|S_k|\times 1}\\
		0_{|S_k|\times 1}
	\end{array}
	\right)
	\end{array}.
\end{equation}
Let $\vt^*$ denote the optimal solution of problem \eqref{obtain_lin_cont}, then we can recover the optimal linear control $v^k = \vt^*_{S_k}$.

{\color{red} END DRAFT}

==> shooting_derivative.tex <==

The execution of our shooting algorithm relies in computing the derivative of the Shooting function. However, since in general each component of the shooting function depend on the initial and final value of the states and costates, this derivative is sensitive to the integration scheme used to integrate the dynamics. 

One approach to perform this computation is to treat the integration step as a black box inside the evaluation of the shooting function and use automatic differentiation to compute the shooting function's derivative. Another is to give an analytical representation of this derivative of interest in terms of the flow of the dynamics of (TP). This introduces the necessity to compute the flow numerically as well. 

Given a Cauchy problem
\begin{equation}
	\label{cauchy_problem}
	\dot{x}_t = f(x_t), \ x(0) = x_0,
\end{equation}
where $f\colon \mathbb{R}^n \to \mathbb{R}^n$ is a $\C^1$ function, we define the flow of system \eqref{cauchy_problem} as the matrix
\begin{equation}
	\label{flow}
	\Psi_t = \frac{\partial x_t}{\partial x_0}.
\end{equation}

Taking time derivatives on both sides of \eqref{flow}, we obtain
\begin{align*}
	\dot{\Psi} 
	& = \frac{\dd }{\dd t}\frac{\partial}{\partial  x_0}x_t = \frac{\partial}{\partial x_0} f(x_t)\\
	& = \frac{\partial f(x_t)}{\partial x} \Psi 
\end{align*}

Clearly we have $\Psi_0 = I_n$, hence computing the flow of the ODE described in \eqref{cauchy_problem} reduces to solving the Cauchy problem given by
\begin{equation}
	\label{flow.cauchy}
	\dot{\Psi} = \frac{\partial f(x_t)}{\partial x} \Psi, \ \Psi_0 = I_n.
\end{equation}

This Cauchy problem can be solved by any numerical scheme desired. 

The next step is to compute the derivative of the shooting function. To simplify notation, let $X_t = \left( \left(x^k(t)\right)_{k=1}^N, \left(p^k(t)\right)_{k=1}^N, \left(T_k\right)_{k=1}^N  \right)$ denote the states from problem (TP), after the control substitutions. Then from equations \eqref{shooting.function.equation} and \eqref{shooting.function.TP}, we note that $\mathcal{S} = \mathcal{S}(X_0, X_1, \beta)$, therefore computing the derivative with respect to the shooting parameters $\nu = (X_0, \beta)$ is reduced to 

\begin{equation}
	\label{shooting.derivative.explicit}
	\mathcal{S}' = 
	\left(
	\begin{array}{cc}
	\disp 
		\underbrace{\frac{\partial\mathcal{S}}{\partial X_0} + \frac{\partial\mathcal{S}}{\partial X_1}\Psi}_{d_{\mathcal{S}} \times d_{TP}} &
	\disp
		\underbrace{\frac{\partial \mathcal{S}}{\partial \beta}}_{d_{\mathcal{S}} \times d_{\beta}}
	\end{array}
	\right).
\end{equation}\footnote{In fact, the shooting function does not depend on the swiching times $(T_k)_{k = 0}^N$. Hence if we take $X_t = \left( \left(x^k(t)\right)_{k=1}^N, \left(p^k(t)\right)_{k=1}^N  \right) $, then the derivative of $\mathcal{S}$ can be expressed as

\begin{equation*}
	\mathcal{S}' = 
	\left(
	\begin{array}{cc}
	\disp 
	\frac{\partial\mathcal{S}}{\partial X_0} + \frac{\partial\mathcal{S}}{\partial X_1}\Psi[0:2nN, :] &
	\disp
	\frac{\partial \mathcal{S}}{\partial \beta}
	\end{array}
	\right).
\end{equation*}

The collums $\Psi[2nN +1: 2nN + N +1]$ are identically null since the states $(T_k)_{k = 0}^N$ have null dynamics.
}
{\color{red} Computing the expression in \eqref{shooting.derivative.explicit} can still prove to be tedious. In this work we (aim to) make this computations symbolicaly with a CAS (Computer Algebra System)}.



